Characterizing the COVID-19 Transmission in South Korea Using the KCDC Patient Data

As the COVID-19 outbreak evolves around the world, the World Health Organization (WHO) and its Member States have been heavily relying on staying at home and lock down measures to control the spread of the virus. In the last months, various signs showed that the COVID-19 curve was flattening, but even the partial lifting of some containment measures (e.g., school closures and telecommuting) appear to favor a second wave of the disease. The accurate evaluation of possible countermeasures and their well-timed revocation are therefore crucial to avoid future waves or reduce their duration. In this paper, we analyze patient and route data of infected patients from January 20, 2020, to May 31, 2020, collected by the Korean Center for Disease Control & Prevention (KCDC). This data analysis helps us to characterize patient mobility patterns and then use this characterization to parameterize simulations to evaluate different what-if scenarios. Although this is not a definitive model of how COVID-19 spreads in a population, its usefulness and flexibility are illustrated using real-world data for exploring virus spread under a variety of circumstances.

==> scenarios.tex <==
% \section{Scenarios and Use-Cases}
% \label{sec:scenario}

% We present three scenarios studying the effect of mobility on COVID-19 virus spreading to show the flexibility of the simulation tool.
% First, we present a worst case scenario, followed by the evaluation of two countermeasures: patient isolation and partial lockdown.
% In the following simulations we consider Seoul's Gangnam district. 
The district's population is 604,586 and there is a total of 7043 buildings. We do not have any information on the number of stories, entries, or rooms within each building. This information is crucial, especially for apartment buildings, where multiple people can be inside the same building at the same time without contact. 
To address this lack of information, we limit the population in our simulations.

% \subsection{Worst Case Scenario}
% \label{worst-case-simulation}


% First, we simulate a worst case scenario where all agents have the same mobility {\em before} and {\em after} infection, i.e., no isolation is practiced.
% Agents only have two states: healthy and infected.
% Fig.~\ref{fig:worst-simulation-results} shows the percentage of infected population as a function of time. 
% We present two experiments with population 10,000 and 20,000, and infection rates ranging from 0.001 to 0.05.
% Generally, the percentage of infected people initially grows exponentially, then it becomes linear, and finally the system saturates (all are infected).
% When a lower infection rate is considered, the virus spreads slower, which indicates the importance of wearing masks and social distancing.
% Increasing the population size (from 10,000 to 20,000), the infection speed is faster, which is expected as the area becomes twice as crowded, see Fig.~\ref{fig:worst-simulation-results}\subref{subfig:worst-pop20k}.
% % Comparing to population 10,000 in Fig.~\ref{fig:worst-simulation-results}\ref{subfig:pop10k},
% % the infection is much faster for population 20,000 shown in  Fig.~\ref{fig:worst-simulation-results}\ref{subfig:pop20k}, because the area is more crowded.

% \begin{figure}[t]
%     \centering    
%         \subfloat[Population = 10,000.]{\label{subfig:worst-pop10k}\includegraphics[scale=0.5]{figs/tmp_results/cdf_exp_covid_worst_pop10000_rate0.01_dist1.pdf}}
%         \hfill
%         \subfloat[Population = 20,000.]{\label{subfig:worst-pop20k}\includegraphics[scale=0.5]{figs/tmp_results/cdf_exp_covid_worst_pop20000_rate0.01_dist1.pdf}}
%     \caption{Percentage of infected agents as a function of time (worst scenario).}
%     \label{fig:worst-simulation-results}
% \end{figure}




\subsection{Simulating Patient Isolation}
\label{sec:symptom-simulation}
In this scenario, we evaluate the importance of limiting patient mobility after infection and first symptoms are observed.
Fig.~\ref{fig:patient_states} shows the transition among patient ``states": a healthy person can be infected, then show symptoms, and finally be isolated.
Recall that for people living in the same domicile, their probability of infection is calculated based on Equation~\ref{eq:infection}.
According to the WHO, it takes 1--14 days to show symptoms after infection~\cite{whoQandA}.
We therefore use a Uniform distribution between 1 and 14 days to transition from infected to symptomatic.
Since there exist irresponsible patients who still move even after showing symptoms, as seen in Fig.~\ref{fig:onset}, we 
 use the CDF in Fig.~\ref{fig:onset}\subref{subfig:onset_date} to determine the number of active days after first symptoms. 
We do not distinguish the behavior of super and low spreaders because of lack of data (there are only two super spreaders with  \textit{symptom\_onset} information available).
After each infected person exhausts their 
 active days after infection, they are isolated (self-quarantine or hospitalization). 
 

Fig.~\ref{fig:symptom-simulation-results} depicts the percentage of infected population for the above scenario.
Comparing these results with the worst case scenario in Fig.~\ref{fig:worst-simulation-results}, the effectiveness of patient isolation is clear. 
Specifically, for infection rate {\bf 0.001}, only {\bf xx}\% of the population is infected in {\bf xx} days (against the {\bf xx}\% observed in the worst case scenario during the same period).
With higher infection rates, and since this scenario allows some mobility after symptoms, the benefit is not as clear as in the case with low infection rates because all of the population gets infected before the benefit of patient isolation takes effect.



As a companion to Fig.~\ref{fig:symptom-simulation-results}, we also present the portions of ``active while infected" and isolated agents, see Fig.~\ref{fig:symptom-simulation-results-active}.
\lishan{
On the one hand, Fig.~\ref{fig:symptom-simulation-results-active}\subref{subfig:symptom-active} shows the percentage of ``active while infected'' patients in the population with infection rate 0.001 and 0.01. The total population simulated here is 10,000. The benefit of patient isolation can be seen: the percentage of active infected population is decreasing after showing a peak, which limits the chance of further infecting others. This is the reason why the total infected population shown in Fig.~\ref{fig:symptom-simulation-results-active}(a)  does not reach 100\% for all the infection rates in Fig.~\ref{fig:worst-simulation-results}\subref{subfig:worst-pop10k} for population 10,000, and infection rate 0.001, 0.003, and 0.005 in Fig.~\ref{fig:worst-simulation-results}\subref{subfig:worst-pop20k} for population 20,000. }\evg{this entire paragraph TBD}
On the other hand, the percentage of isolated population shown in Fig.~\ref{fig:symptom-simulation-results-active}\subref{subfig:symptom-isolated}  explains the decrease of active infected population.
After more agents show symptoms and are isolated, the active infected population starts dropping. 



% \begin{figure*}[tb]
% 	\centering
% 	\begin{minipage}[t]{\textwidth}
% 		\centering
%  		\includegraphics[scale=0.8]{figs/patient_states.png}
% 	\end{minipage}
% % 	\vspace{-\baselineskip}
% % 	\vspace{-1em}
% 	\caption{State transition of agents using different distributions in Simulation Basic+Symptom.}
% 	\label{fig:patient_states}
% % 	\vspace{-1em}
% \end{figure*}


\begin{figure}[t]
    \centering    
        \subfloat[Population = 10,000.]{\label{subfig:symptom-pop10k}\includegraphics[scale=0.5]{figs/tmp_results/newcdf_exp_covid_symptom_pop10000_rate0.005_dist1.pdf}}
        \hfill
        \subfloat[Population = 20,000.]{\label{subfig:symptom-pop20k}\includegraphics[scale=0.5]{figs/tmp_results/newcdf_exp_covid_symptom_pop20000_rate0.005_dist1.pdf}}
        
        \subfloat[Population = 10,000.]{\label{subfig:symptom-pop10k}\includegraphics[scale=0.5]{figs/tmp_results/cdf_exp_covid_symptom_pop10000_rate0.01_dist1.pdf}}
        \hfill
        \subfloat[Population = 20,000.]{\label{subfig:symptom-pop20k}\includegraphics[scale=0.5]{figs/tmp_results/cdf_exp_covid_symptom_pop20000_rate0.01_dist1.pdf}}
    \caption{Percentage of infected population  when simulating patient isolation.}
    \label{fig:symptom-simulation-results}
\end{figure}


\begin{figure}[t]
    \centering    
        \subfloat[Active while infected.]{\label{subfig:symptom-active}\includegraphics[scale=0.5]{figs/tmp_results/active.pdf}}
        \hfill
        \subfloat[Isolated.]{\label{subfig:symptom-isolated}\includegraphics[scale=0.5]{figs/tmp_results/isolation.pdf}}
    \caption{Percentage of active while infected population and the isolated population with 10,000 population simulated in total.}
    \label{fig:symptom-simulation-results-active}
\end{figure}


\IGNORE{
\subsection{Simulating Partial Lockdown}
\label{sec:patial-lockdown-simulation}
Another countermeasure is partial lockdown, i.e., agents are only allowed to travel to a limited distance from their home. 
In this simulation, we use the initial position of each agent as their home address and limit the radius of the active area of an agent.
%There is a restriction on the initial positions: agents are initialized on a road where they can reach at least one building in their limited active area. Otherwise if the active area of an agent is only open air, the chance of infection is negligible, so this agent will never be infected, and there is no need to simulate this agent.
\lishan{
We consider two different distance restrictions: 1 and 2 miles, with population 5,000 and 10,000, and fixed infection rate of 0.006. 
The percentage of infected population as a function of time is shown in Fig.~\ref{fig:distance}. 
When the distance limitation is shorter, the  virus spreads slower.
}

% \begin{enumerate}
%     \item Infection time (or infection rate, as \textit{\#infection}/\textit{infection\_time}) vs. probability of infection. This way, we can see how protections (e.g., masks) can help  reduce the spread of the virus.
%     \item Infection time vs. distance people can travel (e.g., people must stay in their neighborhood or within $N$ km from their initial position).
%     \item What happens (i.e., infection time) if \textit{i)} nobody, \textit{ii)} only contagious users, or \textit{iii)} all infected users are isolated (i.e., they cannot move)? This way, we can look into the importance of testing and quarantine to avoid asymptomatic patients that spread the infection. \lishan{ This is interesting. If (iii), can healthy agents move to the building that has infected users?}
%     \item How does the infection time change if users decide to vaccinate (i.e., they become immune and cannot spread the virus). This may be done by rolling a dice every $N$ cycles (e.g., a day) and inoculating healthy users based on the outcome. Increasing the probability that a user chooses to vaccinate, we can have a look into how many people should vaccinate to stop the contagion.
% \end{enumerate}

% \evg{TBD: What is this useflness of the simulation and this model: we show that Geomeson can be used as a tool to evaluaate different virus spread scenarios and be parameterized with real data. Add the disclaimer that this is not a definitive model of COVID prediction but a flexible model to explore different scenarios. Add this also to abstract, introduction, conclusions.}'







\begin{figure}[t]
    \centering    
        \subfloat[Population = 5,000, infection rate = 0.006]{\label{subfig:distance-pop5k}\includegraphics[scale=0.5]{figs/tmp_results/distance_pop5000_rate0.006.pdf}}
        \hfill
        \subfloat[Population = 10,000, infection rate = 0.006]{\label{subfig:distance-pop10k}\includegraphics[scale=0.5]{figs/tmp_results/distance_pop10000_rate0.006.pdf}}
        
        \subfloat[Population = 10,000, infection rate = 0.006]{\label{subfig:distance-pop10k}\includegraphics[scale=0.5]{figs/tmp_results/distance_pop10000_rate0.006_with_baseline.pdf}}
        
 
    \caption{Percentage of infected population while applying partial lockdown. The simulated infection rate is 0.006.}
    \label{fig:limit-dist-simulation-results}
\end{figure}
}
